The Economics of Blockchain Governance: Evaluate Liquid Democracy on the Internet Computer

Decentralized Autonomous Organizations (DAOs), utilizing blockchain technology to enable collective governance, are a promising innovation. This research addresses the ongoing query in blockchain governance: How can DAOs optimize human cooperation? Focusing on the Network Nervous System (NNS), a comprehensive on-chain governance framework underpinned by the Internet Computer Protocol (ICP) and liquid democracy principles, we employ theoretical abstraction and simulations to evaluate its potential impact on cooperation and economic growth within DAOs. Our findings emphasize the significance of the NNS's staking mechanism, particularly the reward multiplier, in aligning individual short-term interests with the DAO's long-term prosperity. This study contributes to the understanding and effective design of blockchain-based governance systems.

==> figs/fig1.tex <==
\begin{figure}[!htbp]
\centering
\captionsetup{justification=centering}
\includegraphics[width=0.49\textwidth]{figs/nns_feature.png}
    \caption{Network Nervous System (NNS) on the Internet Computer Protocol (ICP).}
    \label{fig: nns}
\end{figure}

==> tabs/tab1.tex <==
\begin{table}[!htbp]
\centering
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{|>{\ttfamily}l|p{7cm}|}
\hline
\textbf{Function} & \textbf{Description} \\ \hline
calculate\_slope\_intercept(f) & Define points \( (x_1, y_1) = (6, 1.06) \) and \( (x_2, y_2) = (96, 2) \). Calculate slope \( m \) and intercept \( b \) for the line segment. Return a wrapper function for \( f \) with parameters \( x, m, b \). \\ \hline
multiplier\_duration(x, m, b) & 
- If \( x < 6 \), return "dissolve delay must be at least 6 months". \newline
- If \( x = 6 \), return 1.06. \newline
- If \( x > 96 \), return 2. \newline
- Otherwise, return \( m \times x + b \). \\ \hline
\end{tabular}}
\caption{Pseudocode for the duration multiplier}
\label{tab: multiplier_duration}
\end{table}



==> tabs/tab2.tex <==
\begin{table}[!htbp]
\centering
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{|>{\ttfamily}l|>{\raggedright\arraybackslash}p{10cm}|}
\hline
\textbf{Function} & \textbf{Description} \\ \hline
Multiplier\_Age(x) & 
Check the value of \( x \): \newline
- If \( x < 0 \), return "the age is out of range". \newline
- If \( x > 48 \), return 1.25. \newline
- Otherwise: \newline
    - Calculate the slope \( m \) as \( 0.25 / 48 \). \newline
    - Set the intercept \( b \) to 1. \newline
    - Return \( m \times x + b \). \\
\hline
\end{tabular}}
\caption{Pseudocode for the Age Multiplier Function}
\label{tab: age_multiplier}
\end{table}
